Wild Berry image dataset collected in Finnish forests and peatlands using drones

Berry picking has long-standing traditions in Finland, yet it is challenging and can potentially be dangerous. The integration of drones equipped with advanced imaging techniques represents a transformative leap forward, optimising harvests and promising sustainable practices. We propose WildBe, the first image dataset of wild berries captured in peatlands and under the canopy of Finnish forests using drones. Unlike previous and related datasets, WildBe includes new varieties of berries, such as bilberries, cloudberries, lingonberries, and crowberries, captured under severe light variations and in cluttered environments. WildBe features 3,516 images, including a total of 18,468 annotated bounding boxes. We carry out a comprehensive analysis of WildBe using six popular object detectors, assessing their effectiveness in berry detection across different forest regions and camera types. WildBe is publicly available on HuggingFace at https://huggingface.co/datasets/FBK-TeV/WildBe.

==> sections/related.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related datasets (1 column)}
\begin{itemize}
\item include and describe similar datasets from drones if there are many, otherwise we can skip this section and put the description only in the introduction
\end{itemize}

==> tables/multi.tex <==
\newcolumntype{g}{>{\columncolor{mygray}}c}
\begin{table}[t!]
\centering
\tabcolsep 3pt
\caption{
Multi-class object detection results evaluated in terms of average precision (AP) and instance-weighted average AP (WAvg).
Key -- Bil.: bilberry, Cloud.: cloudberry, Crow.: crowberry, Lingon.: lingonberry.
Below each berry category, we indicate the number of instances.
}
\label{tab:multi}

\vspace{-3mm}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{rlcccccg}
    \toprule
    & Method & Bil. & Cloud. & Crow. & Lingon. & WAvg \\
    \toprule
    & \color{gray} Instances & \color{gray} 389 & \color{gray} 42 & \small \color{gray} 301 & \color{gray} 233 & \\
    \small \color{gray} 1 & FasterRCNN & 63.8 & 69.0 & 38.5 & 39.3 & 50.2 \\
    \small \color{gray} 2 & VarifocalNet & 69.4 & 73.7 & 44.8 & 50.4 & 57.3 \\
    \small \color{gray} 3 & GLIP & \textbf{71.0} & \textbf{78.7} & \textbf{46.7} & \textbf{54.1} & \textbf{59.7} \\
    \small \color{gray} 4 & DINO & 70.0 & 71.6 & 45.9 & 50.9 & 57.9 \\
    \small \color{gray} 5 & ObjectBox & 66.2 & 73.3 & 43.2 & 46.9 & 54.7 \\
    \small \color{gray} 6 & YOLOv8 & 64.7 & 70.4 & 44.7 & 41.1 & 53.0\\
    \bottomrule
\end{tabular}
}
\end{table}


==> tables/single.tex <==
\newcolumntype{g}{>{\columncolor{mygray}}c}
\begin{table}[t!]
\centering
\tabcolsep 3pt
\caption{
Single-class object detection results evaluated in terms of average precision (AP), AP on small detections ($\textrm{AP}_\textrm{S}$), and AP on medium detections ($\textrm{AP}_\textrm{M}$).
AP on big detections is not shown because no big detections are present.
}
\label{tab:single}

\vspace{-3mm}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{rlccc}
    \toprule
    & Method & AP & $\textrm{AP}_\textrm{S}$ & $\textrm{AP}_\textrm{M}$ \\
    \toprule
    \color{gray} 1 & FasterRCNN & 52.6 & 49.9 & 76.1 \\
    \color{gray} 2 & VarifocalNet & 59.3 & 56.9 & 81.8 \\
    \color{gray} 3 & GLIP & \textbf{60.6} & \textbf{58.0} & \textbf{82.3} \\
    \color{gray} 4 & DINO & 59.6 & 57.5 & 78.1 \\
    \color{gray} 5 & ObjectBox & 55.2 & 52.6 & 77.7 \\
    \color{gray} 6 & YOLOv8 & 56.2 & 53.4 & 79.6 \\
    \bottomrule
\end{tabular}
% }
\end{table}

